Estimates for the restriction of automorphic forms on hyperbolic manifolds to compact geodesic cycles

We find estimates for the restriction of automorphic forms on hyperbolic manifolds to compact geodesic cycles. The geodesic cycles we study are themselves hyperbolic manifolds of lower dimension. The restriction of an automorphic form to such a geodesic cycle can be expanded into eigenfunctions of the Laplacian on the geodesic cycle. We prove exponential decay for the coefficients in this expansion.

==> preambel.tex <==
\usepackage[T1]{fontenc}
\usepackage[ngerman,english]{babel}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{amsxtra}
\usepackage{color}
%\usepackage[breaklinks]{hyperref}
\usepackage{enumitem}
\usepackage{tocloft}
\usepackage{makeidx}
\usepackage{textcomp}
\usepackage{tabularx}
\usepackage{rotating}
\usepackage{multirow}
\usepackage{booktabs,longtable}
\usepackage[all]{xy}
\usepackage{float}

\setenumerate{itemsep=0pt} % topsep=0pt
\setitemize{itemsep=0pt} % topsep=0pt
\setdescription{itemsep=0pt} % topsep=0pt
\setlist{noitemsep}
%\setlength{\itemsep}{0pt}
%\setlength{\parskip}{0pt}
%\setlength{\parsep}{0pt}
%\addtolength{\cftbeforesecskip}{-9pt}
%\renewcommand{\cftsecfont}{\normalfont}

\makeindex

\setcounter{tocdepth}{2}

